StyleRetoucher: Generalized Portrait Image Retouching with GAN Priors

Creating fine-retouched portrait images is tedious and time-consuming even for professional artists. There exist automatic retouching methods, but they either suffer from over-smoothing artifacts or lack generalization ability. To address such issues, we present StyleRetoucher, a novel automatic portrait image retouching framework, leveraging StyleGAN's generation and generalization ability to improve an input portrait image's skin condition while preserving its facial details. Harnessing the priors of pretrained StyleGAN, our method shows superior robustness: a). performing stably with fewer training samples and b). generalizing well on the out-domain data. Moreover, by blending the spatial features of the input image and intermediate features of the StyleGAN layers, our method preserves the input characteristics to the largest extent. We further propose a novel blemish-aware feature selection mechanism to effectively identify and remove the skin blemishes, improving the image skin condition. Qualitative and quantitative evaluations validate the great generalization capability of our method. Further experiments show StyleRetoucher's superior performance to the alternative solutions in the image retouching task. We also conduct a user perceptive study to confirm the superior retouching performance of our method over the existing state-of-the-art alternatives.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> ref_file.tex <==
%%% ====================================================================
%%%  BibTeX-file{
%%%     author         ="Gerry Murray",
%%%     version        ="1.2",
%%%     date           ="2 April 2012",
%%%     filename       ="acmsmall-sample-bibfile.bib",
%%%     address        ="ACM, NY",
%%%     email          ="murray at hq.acm.org",
%%%     codetable      ="ISO/ASCII",
%%%     keywords       ="ACM Reference Format, bibliography, citation, references",
%%%     supported      ="yes",
%%%     docstring      ="This BibTeX database file contains 'bibdata' entries
%%%                        that 'match' the examples provided in the Specifications Document
%%%                        AND, also, 'legacy'-type bibs. It should assist authors in
%%%                        choosing the 'correct' at-bibtype and necessary bib-fields
%%%                        so as to obtain the appropriate ACM Reference Format output.
%%%                        It also contains many 'Standard Abbreviations'. "
%%%  }
%%% ====================================================================

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

%{AMS}
@String{AMSTrans="American Mathematical Society Translations" }
@String{AMSTrans="Amer. Math. Soc. Transl." }
@String{BullAMS="Bulletin of the American Mathematical Society" }
@String{BullAMS="Bull. Amer. Math. Soc." }
@String{ProcAMS="Proceedings of the American Mathematical Society" }
@String{ProcAMS="Proc. Amer. Math. Soc." }
@String{TransAMS="Transactions of the American Mathematical Society" }
@String{TransAMS="Trans. Amer. Math. Soc." }

%ACM
@String{CACM="Communications of the {ACM}" }
@String{CACM="Commun. {ACM}" }
@String{CompServ="Comput. Surveys" }
@String{JACM="J. ACM" }
@String{ACMMathSoft="{ACM} Transactions on Mathematical Software" }
@String{ACMMathSoft="{ACM} Trans. Math. Software" }
@String{SIGNUM="{ACM} {SIGNUM} Newsletter" }
@String{SIGNUM="{ACM} {SIGNUM} Newslett." }

@String{AmerSocio="American Journal of Sociology" }
@String{AmerStatAssoc="Journal of the American Statistical Association" }
@String{AmerStatAssoc="J. Amer. Statist. Assoc." }
@String{ApplMathComp="Applied Mathematics and Computation" }
@String{ApplMathComp="Appl. Math. Comput." }
@String{AmerMathMonthly="American Mathematical Monthly" }
@String{AmerMathMonthly="Amer. Math. Monthly" }
@String{BIT="{BIT}" }
@String{BritStatPsych="British Journal of Mathematical and Statistical
  Psychology" }
@String{BritStatPsych="Brit. J. Math. Statist. Psych." }
@String{CanMathBull="Canadian Mathematical Bulletin" }
@String{CanMathBull="Canad. Math. Bull." }
@String{CompApplMath="Journal of Computational and Applied Mathematics" }
@String{CompApplMath="J. Comput. Appl. Math." }
@String{CompPhys="Journal of Computational Physics" }
@String{CompPhys="J. Comput. Phys." }
@String{CompStruct="Computers and Structures" }
@String{CompStruct="Comput. \& Structures" }
@String{CompJour="The Computer Journal" }
@String{CompJour="Comput. J." }
@String{CompSysSci="Journal of Computer and System Sciences" }
@String{CompSysSci="J. Comput. System Sci." }
@String{Computing="Computing" }
@String{ContempMath="Contemporary Mathematics" }
@String{ContempMath="Contemp. Math." }
@String{Crelle="Crelle's Journal" }
@String{GiornaleMath="Giornale di Mathematiche" }
@String{GiornaleMath="Giorn. Mat." } % didn't find in AMS MR., ibid.

%IEEE
@String{Computer="{IEEE} Computer" }
@String{IEEETransComp="{IEEE} Transactions on Computers" }
@String{IEEETransComp="{IEEE} Trans. Comput." }
@String{IEEETransAC="{IEEE} Transactions on Automatic Control" }
@String{IEEETransAC="{IEEE} Trans. Automat. Control" }
@String{IEEESpec="{IEEE} Spectrum" } % didn't find in AMS MR
@String{ProcIEEE="Proceedings of the {IEEE}" }
@String{ProcIEEE="Proc. {IEEE}" } % didn't find in AMS MR
@String{IEEETransAeroElec="{IEEE} Transactions on Aerospace and Electronic
Systems" }
@String{IEEETransAeroElec="{IEEE} Trans. Aerospace Electron. Systems" }

@String{IMANumerAna="{IMA} Journal of Numerical Analysis" }
@String{IMANumerAna="{IMA} J. Numer. Anal." }
@String{InfProcLet="Information Processing Letters" }
@String{InfProcLet="Inform. Process. Lett." }
@String{InstMathApp="Journal of the Institute of Mathematics and
  its Applications" }
@String{InstMathApp="J. Inst. Math. Appl." }
@String{IntControl="International Journal of Control" }
@String{IntControl="Internat. J. Control" }
@String{IntNumerEng="International Journal for Numerical Methods in
  Engineering" }
@String{IntNumerEng="Internat. J. Numer. Methods Engrg." }
@String{IntSuper="International Journal of Supercomputing Applications" }
@String{IntSuper="Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
@String{Kibernetika="Kibernetika" }
@String{JResNatBurStand="Journal of Research of the National Bureau
  of Standards" }
@String{JResNatBurStand="J. Res. Nat. Bur. Standards" }
@String{LinAlgApp="Linear Algebra and its Applications" }
@String{LinAlgApp="Linear Algebra Appl." }
@String{MathAnaAppl="Journal of Mathematical Analysis and Applications" }
@String{MathAnaAppl="J. Math. Anal. Appl." }
@String{MathAnnalen="Mathematische Annalen" }
@String{MathAnnalen="Math. Ann." }
@String{MathPhys="Journal of Mathematical Physics" }
@String{MathPhys="J. Math. Phys." }
@String{MathComp="Mathematics of Computation" }
@String{MathComp="Math. Comp." }
@String{MathScand="Mathematica Scandinavica" }
@String{MathScand="Math. Scand." }
@String{TablesAidsComp="Mathematical Tables and Other Aids to Computation" }
@String{TablesAidsComp="Math. Tables Aids Comput." }
@String{NumerMath="Numerische Mathematik" }
@String{NumerMath="Numer. Math." }
@String{PacificMath="Pacific Journal of Mathematics" }
@String{PacificMath="Pacific J. Math." }
@String{ParDistComp="Journal of Parallel and Distributed Computing" }
@String{ParDistComp="J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
@String{ParComputing="Parallel Computing" }
@String{ParComputing="Parallel Comput." }
@String{PhilMag="Philosophical Magazine" }
@String{PhilMag="Philos. Mag." }
@String{ProcNAS="Proceedings of the National Academy of Sciences
  of the USA" }
@String{ProcNAS="Proc. Nat. Acad. Sci. U. S. A." }
@String{Psychometrika="Psychometrika" }
@String{QuartMath="Quarterly Journal of Mathematics, Oxford, Series (2)" }
@String{QuartMath="Quart. J. Math. Oxford Ser. (2)" }
@String{QuartApplMath="Quarterly of Applied Mathematics" }
@String{QuartApplMath="Quart. Appl. Math." }
@String{RevueInstStat="Review of the International Statisical Institute" }
@String{RevueInstStat="Rev. Inst. Internat. Statist." }

%SIAM
@String{JSIAM="Journal of the Society for Industrial and Applied
  Mathematics" }
@String{JSIAM="J. Soc. Indust. Appl. Math." }
@String{JSIAMB="Journal of the Society for Industrial and Applied
  Mathematics, Series B, Numerical Analysis" }
@String{JSIAMB="J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
@String{SIAMAlgMeth="{SIAM} Journal on Algebraic and Discrete Methods" }
@String{SIAMAlgMeth="{SIAM} J. Algebraic Discrete Methods" }
@String{SIAMAppMath="{SIAM} Journal on Applied Mathematics" }
@String{SIAMAppMath="{SIAM} J. Appl. Math." }
@String{SIAMComp="{SIAM} Journal on Computing" }
@String{SIAMComp="{SIAM} J. Comput." }
@String{SIAMMatrix="{SIAM} Journal on Matrix Analysis and Applications" }
@String{SIAMMatrix="{SIAM} J. Matrix Anal. Appl." }
@String{SIAMNumAnal="{SIAM} Journal on Numerical Analysis" }
@String{SIAMNumAnal="{SIAM} J. Numer. Anal." }
@String{SIAMReview="{SIAM} Review" }
@String{SIAMReview="{SIAM} Rev." }
@String{SIAMSciStat="{SIAM} Journal on Scientific and Statistical
Computing" }
@String{SIAMSciStat="{SIAM} J. Sci. Statist. Comput." }

@String{SoftPracExp="Software Practice and Experience" }
@String{SoftPracExp="Software Prac. Experience" } % didn't find in AMS MR
@String{StatScience="Statistical Science" }
@String{StatScience="Statist. Sci." }
@String{Techno="Technometrics" }
@String{USSRCompMathPhys="{USSR} Computational Mathematics and Mathematical
Physics" }
@String{USSRCompMathPhys="{U. S. S. R.} Comput. Math. and Math. Phys." }
@String{VLSICompSys="Journal of {VLSI} and Computer Systems" }
@String{VLSICompSys="J. {VLSI} Comput. Syst." }
@String{ZAngewMathMech="Zeitschrift fur Angewandte Mathematik und
  Mechanik" }
@String{ZAngewMathMech="Z. Angew. Math. Mech." }
@String{ZAngewMathPhys="Zeitschrift fur Angewandte Mathematik und Physik" }
@String{ZAngewMathPhys="Z. Angew. Math. Phys." }

% Publishers % ================================================= |

@String{Academic="Academic Press" }
@String{ACMPress="{ACM} Press" }
@String{AdamHilger="Adam Hilger" }
@String{AddisonWesley="Addison-Wesley" }
@String{AllynBacon="Allyn and Bacon" }
@String{AMS="American Mathematical Society" }
@String{Birkhauser="Birkha{\"u}ser" }
@String{CambridgePress="Cambridge University Press" }
@String{Chelsea="Chelsea" }
@String{ClaredonPress="Claredon Press" }
@String{DoverPub="Dover Publications" }
@String{Eyolles="Eyolles" }
@String{HoltRinehartWinston="Holt, Rinehart and Winston" }
@String{Interscience="Interscience" }
@String{JohnsHopkinsPress="The Johns Hopkins University Press" }
@String{JohnWileySons="John Wiley and Sons" }
@String{Macmillan="Macmillan" }
@String{MathWorks="The Math Works Inc." }
@String{McGrawHill="McGraw-Hill" }
@String{NatBurStd="National Bureau of Standards" }
@String{NorthHolland="North-Holland" }
@String{OxfordPress="Oxford University Press" }  %address Oxford or London?
@String{PergamonPress="Pergamon Press" }
@String{PlenumPress="Plenum Press" }
@String{PrenticeHall="Prentice-Hall" }
@String{SIAMPub="{SIAM} Publications" }
@String{TexasPress="University of Texas Press" }
@String{VanNostrand="Van Nostrand" }
@String{WHFreeman="W. H. Freeman and Co." }

%Entries

@article{wang2022panini,
  title={Panini-Net: GAN Prior Based Degradation-Aware Feature Interpolation for Face Restoration},
  author={Wang, Yinhuai and Hu, Yujie and Zhang, Jian},
  journal={arXiv preprint arXiv:2203.08444},
  year={2022}
}

@inproceedings{karras2019style,
  title={A style-based generator architecture for generative adversarial networks},
  author={Karras, Tero and Laine, Samuli and Aila, Timo},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={4401--4410},
  year={2019}
}

@inproceedings{menon2020pulse,
  title={Pulse: Self-supervised photo upsampling via latent space exploration of generative models},
  author={Menon, Sachit and Damian, Alexandru and Hu, Shijia and Ravi, Nikhil and Rudin, Cynthia},
  booktitle={Proceedings of the ieee/cvf conference on computer vision and pattern recognition},
  pages={2437--2445},
  year={2020}
}

@inproceedings{chan2021glean,
  title={Glean: Generative latent bank for large-factor image super-resolution},
  author={Chan, Kelvin CK and Wang, Xintao and Xu, Xiangyu and Gu, Jinwei and Loy, Chen Change},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={14245--14254},
  year={2021}
}

@inproceedings{wang2021towards,
  title={Towards real-world blind face restoration with generative facial prior},
  author={Wang, Xintao and Li, Yu and Zhang, Honglun and Shan, Ying},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9168--9178},
  year={2021}
}

@inproceedings{yang2021gan,
  title={Gan prior embedded network for blind face restoration in the wild},
  author={Yang, Tao and Ren, Peiran and Xie, Xuansong and Zhang, Lei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={672--681},
  year={2021}
}

@inproceedings{wu2021stylespace,
  title={Stylespace analysis: Disentangled controls for stylegan image generation},
  author={Wu, Zongze and Lischinski, Dani and Shechtman, Eli},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12863--12872},
  year={2021}
}

@inproceedings{velusamy2020fabsoften,
  title={FabSoften: Face beautification via dynamic skin smoothing, guided feathering, and texture restoration},
  author={Velusamy, Sudha and Parihar, Rishubh and Kini, Raviprasad and Rege, Aniket},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={530--531},
  year={2020}
}

@inproceedings{zhang2014100,
  title={100+ times faster weighted median filter (WMF)},
  author={Zhang, Qi and Xu, Li and Jia, Jiaya},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2830--2837},
  year={2014}
}

@inproceedings{tomasi1998bilateral,
  title={Bilateral filtering for gray and color images},
  author={Tomasi, Carlo and Manduchi, Roberto},
  booktitle={Sixth international conference on computer vision (IEEE Cat. No. 98CH36271)},
  pages={839--846},
  year={1998},
  organization={IEEE}
}

@inproceedings{xu2011image,
  title={Image smoothing via L 0 gradient minimization},
  author={Xu, Li and Lu, Cewu and Xu, Yi and Jia, Jiaya},
  booktitle={Proceedings of the 2011 SIGGRAPH Asia conference},
  pages={1--12},
  year={2011}
}

@article{min2014fast,
  title={Fast global image smoothing based on weighted least squares},
  author={Min, Dongbo and Choi, Sunghwan and Lu, Jiangbo and Ham, Bumsub and Sohn, Kwanghoon and Do, Minh N},
  journal={IEEE Transactions on Image Processing},
  volume={23},
  number={12},
  pages={5638--5653},
  year={2014},
  publisher={IEEE}
}

@incollection{gastal2011domain,
  title={Domain transform for edge-aware image and video processing},
  author={Gastal, Eduardo SL and Oliveira, Manuel M},
  booktitle={ACM SIGGRAPH 2011 papers},
  pages={1--12},
  year={2011}
}

@inproceedings{guo2017mutually,
  title={Mutually guided image filtering},
  author={Guo, Xiaojie and Li, Yu and Ma, Jiayi},
  booktitle={Proceedings of the 25th ACM international conference on Multimedia},
  pages={1283--1290},
  year={2017}
}

@inproceedings{liang2015facemore,
  title={FaceMore: A face beautification platform on the cloud},
  author={Liang, Lingyu and Liu, Deng and Jin, Lianwen},
  booktitle={2015 IEEE International Conference on Systems, Man, and Cybernetics},
  pages={1798--1803},
  year={2015},
  organization={IEEE}
}

@article{lin2019exemplar,
  title={Exemplar-based freckle retouching and skin tone adjustment},
  author={Lin, Tsung-Ying and Tsai, Yu-Ting and Huang, Tsung-Shian and Lin, Wen-Chieh and Chuang, Jung-Hong},
  journal={Computers \& Graphics},
  volume={78},
  pages={54--63},
  year={2019},
  publisher={Elsevier}
}

@article{cai2018learning,
  title={Learning a deep single image contrast enhancer from multi-exposure images},
  author={Cai, Jianrui and Gu, Shuhang and Zhang, Lei},
  journal={IEEE Transactions on Image Processing},
  volume={27},
  number={4},
  pages={2049--2062},
  year={2018},
  publisher={IEEE}
}

@inproceedings{deng2018aesthetic,
  title={Aesthetic-driven image enhancement by adversarial learning},
  author={Deng, Yubin and Loy, Chen Change and Tang, Xiaoou},
  booktitle={Proceedings of the 26th ACM international conference on Multimedia},
  pages={870--878},
  year={2018}
}

@inproceedings{he2020conditional,
  title={Conditional sequential modulation for efficient global image retouching},
  author={He, Jingwen and Liu, Yihao and Qiao, Yu and Dong, Chao},
  booktitle={European Conference on Computer Vision},
  pages={679--695},
  year={2020},
  organization={Springer}
}

@InProceedings{Shafaei2021WACV,
    author    = {Shafaei, Alireza and Little, James J. and Schmidt, Mark},
    title     = {AutoRetouch: Automatic Professional Face Retouching},
    booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV)},
    month     = {January},
    year      = {2021},
    pages     = {990-998}
}

@inproceedings{NIPS2014_5ca3e9b1,
 author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {Z. Ghahramani and M. Welling and C. Cortes and N. Lawrence and K.Q. Weinberger},
 % pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Generative Adversarial Nets},
 % url = {https://proceedings.neurips.cc/paper/2014/file/5ca3e9b122f61f8f06494c97b1afccf3-Paper.pdf},
 volume = {27},
 year = {2014}
}


@article{shih2014portrait,
  title={Style transfer for headshot portraits},
  author={Shih, YiChang and Paris, Sylvain and Barnes, Connelly and Freeman, William T and Durand, Fredo},
  journal={ACM Trans. Graph},
  year={2014},
  publisher={ACM}
}

@article{gatys2015neural,
  title={A neural algorithm of artistic style},
  author={Gatys, Leon A and Ecker, Alexander S and Bethge, Matthias},
  journal={arXiv preprint arXiv:1508.06576},
  year={2015}
}

@article{ulyanov2016texture,
  title={Texture networks: Feed-forward synthesis of textures and stylized images},
  author={Ulyanov, Dmitry and Lebedev, Vadim and Vedaldi, Andrea and Lempitsky, Victor},
  journal={arXiv preprint arXiv:1603.03417},
  year={2016}
}

@inproceedings{johnson2016perceptual,
  title={Perceptual losses for real-time style transfer and super-resolution},
  author={Johnson, Justin and Alahi, Alexandre and Fei-Fei, Li},
  booktitle={European conference on computer vision},
  pages={694--711},
  year={2016},
  organization={Springer}
}

@inproceedings{lei2022abpn,
  title={ABPN: Adaptive Blend Pyramid Network for Real-Time Local Retouching of Ultra High-Resolution Photo},
  author={Lei, Biwen and Guo, Xiefan and Yang, Hongyu and Cui, Miaomiao and Xie, Xuansong and Huang, Di},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2108--2117},
  year={2022}
}

@inproceedings{chong2022jojogan,
  title={Jojogan: One shot face stylization},
  author={Chong, Min Jin and Forsyth, David},
  booktitle={European Conference on Computer Vision},
  pages={128--152},
  year={2022},
  organization={Springer}
}


@article{song2021agilegan,
  title={AgileGAN: stylizing portraits by inversion-consistent transfer learning},
  author={Song, Guoxian and Luo, Linjie and Liu, Jing and Ma, Wan-Chun and Lai, Chunpong and Zheng, Chuanxia and Cham, Tat-Jen},
  journal={ACM Transactions on Graphics (TOG)},
  volume={40},
  number={4},
  pages={1--13},
  year={2021},
  publisher={ACM New York, NY, USA}
}


@article{pinkney2020resolution,
  title={Resolution dependent gan interpolation for controllable image synthesis between domains},
  author={Pinkney, Justin NM and Adler, Doron},
  journal={arXiv preprint arXiv:2010.05334},
  year={2020}
}

@article{cao2018cari,
    title={CariGANs: Unpaired Photo-to-Caricature Translation},
    author={Cao, Kaidi and Liao, Jing and Yuan, Lu},
    journal={ACM Transactions on Graphics (Proc. of Siggraph Asia 2018)},
    year={2018}
}

@inproceedings{xia2020joint,
  title={Joint bilateral learning for real-time universal photorealistic style transfer},
  author={Xia, Xide and Zhang, Meng and Xue, Tianfan and Sun, Zheng and Fang, Hui and Kulis, Brian and Chen, Jiawen},
  booktitle={European Conference on Computer Vision},
  pages={327--342},
  year={2020},
  organization={Springer}
}

@inproceedings{wang2019underexposed,
  title={Underexposed photo enhancement using deep illumination estimation},
  author={Wang, Ruixing and Zhang, Qing and Fu, Chi-Wing and Shen, Xiaoyong and Zheng, Wei-Shi and Jia, Jiaya},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={6849--6857},
  year={2019}
}

@inproceedings{zhang2019deep,
  title={Deep exemplar-based video colorization},
  author={Zhang, Bo and He, Mingming and Liao, Jing and Sander, Pedro V and Yuan, Lu and Bermak, Amine and Chen, Dong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8052--8061},
  year={2019}
}

@article{gharbi2017deep,
  title={Deep bilateral learning for real-time image enhancement},
  author={Gharbi, Micha{\"e}l and Chen, Jiawen and Barron, Jonathan T and Hasinoff, Samuel W and Durand, Fr{\'e}do},
  journal={ACM Transactions on Graphics (TOG)},
  volume={36},
  number={4},
  pages={1--12},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@article{he2020condition,
  title={Conditional sequential modulation for efficient global image retouching},
  author={He, Jingwen and Liu, Yihao and Qiao, Yu and Dong, Chao},
  booktitle={European Conference on Computer Vision},
  pages={679--695},
  year={2020},
  organization={Springer}
}

@article{zeng2020learning,
  title={Learning image-adaptive 3d lookup tables for high performance photo enhancement in real-time},
  author={Zeng, Hui and Cai, Jianrui and Li, Lida and Cao, Zisheng and Zhang, Lei},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2020},
  publisher={IEEE}
}

@inproceedings{afifi2021histogan,
  title={Histogan: Controlling colors of gan-generated and real images via color histograms},
  author={Afifi, Mahmoud and Brubaker, Marcus A and Brown, Michael S},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={7941--7950},
  year={2021}
}

@inproceedings{wang2021real,
  title={Real-time image enhancer via learnable spatial-aware 3d lookup tables},
  author={Wang, Tao and Li, Yong and Peng, Jingyang and Ma, Yipeng and Wang, Xian and Song, Fenglong and Yan, Youliang},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2471--2480},
  year={2021}
}

@article{he2019progressive,
  title={Progressive color transfer with dense semantic correspondences},
  author={He, Mingming and Liao, Jing and Chen, Dongdong and Yuan, Lu and Sander, Pedro V},
  journal={ACM Transactions on Graphics (TOG)},
  volume={38},
  number={2},
  pages={1--18},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{abdal2019image2stylegan,
  title={Image2stylegan: How to embed images into the stylegan latent space?},
  author={Abdal, Rameen and Qin, Yipeng and Wonka, Peter},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={4432--4441},
  year={2019}
}

@inproceedings{abdal2020image2styleganpp,
  title={Image2StyleGAN++: How to Edit the Embedded Images?},
  author={Abdal, Rameen and Qin, Yipeng and Wonka, Peter},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8296--8305},
  year={2020}
}

@article{creswell2018inverting,
  title={Inverting the generator of a generative adversarial network},
  author={Creswell, Antonia and Bharath, Anil Anthony},
  journal={IEEE transactions on neural networks and learning systems},
  volume={30},
  number={7},
  pages={1967--1974},
  year={2018},
  publisher={IEEE}
}

@article{richardson2020encoding,
  title={Encoding in style: a stylegan encoder for image-to-image translation},
  author={Richardson, Elad and Alaluf, Yuval and Patashnik, Or and Nitzan, Yotam and Azar, Yaniv and Shapiro, Stav and Cohen-Or, Daniel},
  journal={arXiv preprint arXiv:2008.00951},
  year={2020}
}

@article{zhu2020domain,
  title={In-domain gan inversion for real image editing},
  author={Zhu, Jiapeng and Shen, Yujun and Zhao, Deli and Zhou, Bolei},
  journal={arXiv preprint arXiv:2004.00049},
  year={2020}
}

@article{su2022drawinginstyles,
    author = {Su, Wanchao and Ye, Hui and Chen, Shu-Yu and Gao, Lin and Fu, Hongbo},
    title = {DrawingInStyles: Portrait Image Generation and Editing with Spatially Conditioned StyleGAN},
    journal = {IEEE Transactions on Visualization and Computer Graphics},
    year = {2022},
    publisher={IEEE} 
}

@article{chen2022sofgan,
    title={Sofgan: A portrait image generator with dynamic styling},
    author={Chen, Anpei and Liu, Ruiyang and Xie, Ling and Chen, Zhang and Su, Hao and Yu, Jingyi},
    journal={ACM Transactions on Graphics (TOG)},
    volume={41},
    number={1},
    pages={1--26},
    year={2022},
    publisher={ACM New York, NY}
}

@inproceedings{Karras2019stylegan2,
  title     = {Analyzing and Improving the Image Quality of {StyleGAN}},
  author    = {Tero Karras and Samuli Laine and Miika Aittala and Janne Hellsten and Jaakko Lehtinen and Timo Aila},
  booktitle = {Proc. CVPR},
  year      = {2020}
}

@article{mittal2012making,
  title={Making a “completely blind” image quality analyzer},
  author={Mittal, Anish and Soundararajan, Rajiv and Bovik, Alan C},
  journal={IEEE Signal processing letters},
  volume={20},
  number={3},
  pages={209--212},
  year={2012},
  publisher={IEEE}
}

@article{heusel2017gans,
  title={Gans trained by a two time-scale update rule converge to a local nash equilibrium},
  author={Heusel, Martin and Ramsauer, Hubert and Unterthiner, Thomas and Nessler, Bernhard and Hochreiter, Sepp},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}


@article{tov2021designing,
  title={Designing an encoder for stylegan image manipulation},
  author={Tov, Omer and Alaluf, Yuval and Nitzan, Yotam and Patashnik, Or and Cohen-Or, Daniel},
  journal={ACM Transactions on Graphics (TOG)},
  volume={40},
  number={4},
  pages={1--14},
  year={2021},
  publisher={ACM New York, NY, USA}
}


@inproceedings{patashnik2021styleclip,
  title={Styleclip: Text-driven manipulation of stylegan imagery},
  author={Patashnik, Or and Wu, Zongze and Shechtman, Eli and Cohen-Or, Daniel and Lischinski, Dani},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2085--2094},
  year={2021}
}

@article{harkonen2020ganspace,
  title={Ganspace: Discovering interpretable gan controls},
  author={H{\"a}rk{\"o}nen, Erik and Hertzmann, Aaron and Lehtinen, Jaakko and Paris, Sylvain},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={9841--9850},
  year={2020}
}

@article{abdal2021styleflow,
  title={Styleflow: Attribute-conditioned exploration of stylegan-generated images using conditional continuous normalizing flows},
  author={Abdal, Rameen and Zhu, Peihao and Mitra, Niloy J and Wonka, Peter},
  journal={ACM Transactions on Graphics (ToG)},
  volume={40},
  number={3},
  pages={1--21},
  year={2021},
  publisher={ACM New York, NY}
}

@article{gal2022stylegan,
  title={Stylegan-nada: Clip-guided domain adaptation of image generators},
  author={Gal, Rinon and Patashnik, Or and Maron, Haggai and Bermano, Amit H and Chechik, Gal and Cohen-Or, Daniel},
  journal={ACM Transactions on Graphics (TOG)},
  volume={41},
  number={4},
  pages={1--13},
  year={2022},
  publisher={ACM New York, NY, USA}
}

@inproceedings{zhang2018perceptual,
  title={The Unreasonable Effectiveness of Deep Features as a Perceptual Metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={CVPR},
  year={2018}
}

@article{wang2004image,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P},
  journal={IEEE transactions on image processing},
  volume={13},
  number={4},
  pages={600--612},
  year={2004},
  publisher={IEEE}
}


@inproceedings{wang2018pix2pixHD,
  title={High-Resolution Image Synthesis and Semantic Manipulation with Conditional GANs},
  author={Ting-Chun Wang and Ming-Yu Liu and Jun-Yan Zhu and Andrew Tao and Jan Kautz and Bryan Catanzaro},  
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2018}
}

@misc{ola2008pixlr,
    title        = {Pixlr},
    author       = {Ola Sevandersson},
    year         = 2008,
    note         = {\url{https://www.pixlr.com/}}
}

@misc{meitu2013meitu,
    title        = {MeituPic},
    author       = {Meitu Inc.},
    year         = 2013,
    note         = {\url{http://xiuxiu.meitu.com/}}
}

@misc{beautycam2013meitu,
    title        = {BeautyCam},
    author       = {Meitu Inc.},
    year         = 2013,
    note         = {\url{https://meiyan.meipai.com}}
}

@inproceedings{liu2019stgan,
  title={Stgan: A unified selective transfer network for arbitrary image attribute editing},
  author={Liu, Ming and Ding, Yukang and Xia, Min and Liu, Xiao and Ding, Errui and Zuo, Wangmeng and Wen, Shilei},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={3673--3682},
  year={2019}
}

@article{cho2014properties,
  title={On the properties of neural machine translation: Encoder-decoder approaches},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Bahdanau, Dzmitry and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1409.1259},
  year={2014}
}

@article{yang2022vtoonify,
  title={VToonify: Controllable High-Resolution Portrait Video Style Transfer},
  author={Yang, Shuai and Jiang, Liming and Liu, Ziwei and Loy, Chen Change},
  journal={ACM Transactions on Graphics (TOG)},
  volume={41},
  number={6},
  pages={1--15},
  year={2022},
  publisher={ACM New York, NY, USA}
}
